Generative Deduplication For Socia Media Data Selection

Social media data exhibits severe redundancy caused by its noisy nature. It leads to increased training time and model bias in its processing. To address this issue, we propose a novel Generative Deduplication framework for social media data selection by removing semantically duplicate data. While related work involves data selection in task-specific training, our model acts as an efficient pre-processing method to universally enhance social media NLP pipelines. Specifically, we train a generative model via self-supervised learning to predict a keyword to capture the semantics of noisy social media text for deduplication. Meanwhile, time-dimensional Gaussian noise is added to improve training complexity and avoid learning trivial features. Extensive experiments suggest that our model can better reduce training samples while improving performance than baselines. The results show our model's potential to broadly advance social media language understanding in effectiveness and efficiency.

==> figure_dedup_raw_bar.tex <==
\begin{figure}[ht]
    \centering
    % , trim = {0 10 0 0}
    \includegraphics[width=1.0\textwidth]{figures/deduplication_comparison.pdf}
    \caption{A bar plot shows each dataset's deduplicated training samples for different deduplication approaches. The percentage represents the deduplication ratio compared to the raw data. A smaller ratio indicates a stronger deduplication ability.}
    \label{figure_dedup_raw_bar}
\end{figure}

==> figure_dedup_time.tex <==
\begin{figure*}[ht]
    \centering
    % , trim = {0 10 0 0}
    \includegraphics[width=0.98\textwidth]{figures/dedup_time.pdf}
    \caption{Dedupliaction time of different deduplication approaches. $y$-axis indicates the deduplication time (seconds). \textit{generative} stands for the proposed generative deduplication. \textit{shingles} denotes shingles deduplication. \textit{pairwise} represents the pairwise semantic deduplication. }
    \label{figure_dedup_time}
\end{figure*}

==> rubbish.tex <==
\section{Deduplication Time}
\label{appendix_deduplication_time}
\input{figure_dedup_time}

Figure \ref{figure_dedup_time} presents the deduplication time of different deduplication approaches. We can find that pairwise semantic deduplication takes much longer compared to other methods. The proposed generative deduplication is comparable to shingles deduplication, but it performs better in larger datasets like Emoji and Sentiment in terms of efficiency.


==> table_downstream.tex <==

\begin{table*}[]
\small
\centering
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
Model & MR & CR & SUBJ & MPQA & SST2 & TREC & MRPC & Avg. \\

\midrule
\midrule
GloVe $\dagger$ & $77.25$ & $78.30$ &  $91.17$ &  $87.85$ & $80.18$ &  $83.00$ & $72.87$ &  $81.52$ \\ 
Skip-thought $\ddagger$ & $76.50$ & $80.10$ & $93.60$ & $87.10$ &  $82.00$ & $92.20$ & $73.00$ & $83.50$ \\

Avg. BERT $\dagger$ & $78.66$ & $86.25$ & $94.37$ & $88.66$ &  $84.40$ & $92.80$ & $69.54$ & $84.94$ \\

BERT-CLS $\dagger$ & $78.68$ & $84.85$ & $94.21$ & $88.23$ & $84.13$ & $91.40$ & $71.13$ & $84.66$ \\

IS-BERT $\ddagger$ & $81.09$ & $87.18$ & $94.96$ & $88.75$ & $85.96$  & $88.64$ & $74.24$ &  $85.83$ \\

SimCSE-RoBERTa $\clubsuit$ & $83.37$ & $87.76$ & $95.05$ & $87.16$ & $89.02$ & $90.80$ & $75.13$ &  $86.90$ \\
DiffCSE-RoBERTa $\diamondsuit$ & $82.82$ & $88.61$ & $94.32$ & $87.71$ & $88.63$ & $90.40$ & $\mathbf{76.81}$ & $87.04$ \\

SimCSE-LLaMA $\star$ & $90.42$ & $92.89$ & $95.98$ & $91.37$ & $95.13$ & $95.40$ & $75.12$ & $91.06$ \\
\midrule
AnglE-LLaMA (ours) & $\mathbf{90.90}$ & $\mathbf{93.54}$ & $\mathbf{96.47}$ & $\mathbf{91.50}$ & $\mathbf{95.28}$ & $\mathbf{96.40}$ & $75.36$ & $\mathbf{91.38}$ \\
\bottomrule

\end{tabular}
\end{threeparttable}
\caption{Sentence embeddings for downstream tasks. The reported metrics is accuracy. $\dagger$: results from \citet{sbert-nils-2019}; $\ddagger$: results from \citet{zhang-etal-2020-unsupervised}; $\clubsuit$: results from \citet{simcse_gao_2021}; $\diamondsuit$: results from \citet{chuang-etal-2022-diffcse}; $\star$: results are our implementation using the official code.}
\label{table_downstream}
\end{table*}
